Data-efficient visuomotor policy training using reinforcement learning and generative models

We present a data-efficient framework for solving visuomotor sequential decision-making problems which exploits the combination of reinforcement learning (RL) and latent variable generative models. Our framework trains deep visuomotor policies by introducing an action latent variable such that the feed-forward policy search can be divided into three parts: (i) training a sub-policy that outputs a distribution over the action latent variable given a state of the system, (ii) unsupervised training of a generative model that outputs a sequence of motor actions conditioned on the latent action variable, and (iii) supervised training of the deep visuomotor policy in an end-to-end fashion. Our approach enables safe exploration and alleviates the data-inefficiency problem as it exploits prior knowledge about valid sequences of motor actions. Moreover, we provide a set of measures for evaluation of generative models such that we are able to predict the performance of the RL policy training prior to the actual training on a physical robot. We define two novel measures of disentanglement and local linearity for assessing the quality of latent representations, and complement them with existing measures for assessment of the learned distribution. We experimentally determine the characteristics of different generative models that have the most influence on performance of the final policy training on a robotic picking task.

==> inputs/reserved.tex <==
\begin{figure}
\centering
\begin{minipage}{.4\textwidth}
  \centering
  \includegraphics[height=.7\linewidth]{figures/MMDalpha10_basecolorsGroup11_disentanglement_scores_dict_1589354519359854.png}
  \captionof{figure}{Policy training}
  \label{fig:test1}
\end{minipage}%
\hspace{0cm}
\begin{minipage}{.4\textwidth}
  \centering
  \includegraphics[height=0.7\linewidth]{figures/MMDalpha10_basecolorsGroup21_disentanglement_scores_dict_1589354519359854.png}
  \captionof{figure}{Disentanglement score}
  \label{fig:test2}
\end{minipage}
\end{figure}

==> inputs/todo.tex <==
\section{TODO list}
\paragraph{Final comments}
\begin{itemize}

\item Eq, Sec, Fig vs Equation, Section, Figure
%\item : vs , before align environment
\item action latent variable vs latent action variable
\item KL, DKL, KL-divergence?
\item Explicit naming of authors in the first part of the related work, why?
\item When we have expected values it is not mathematically correct to write neither $\mathbb{E}_{\alpha ~p(.)}[x]$ (not clear what is the dot) nor $\mathbb{E}_{\alpha ~p(alpha)}[x]$ (the left hand side $\alpha$ is a concrete sample while the right hand side one is a function variable). I would therefore suggest to kill the explicit sampling from the notation and always write $\mathbb{E}_{p(\alpha)}[x]$. It is a standard way to denote expectations in the statistics i believe.
\item In section GANs, we say that we use InfoGAN because it encouranges the disentanglement. However, we do not mention it in VAEs even though we do use a higher $\beta$ which encouranges disentanglement. I think we should have a sentence about it there as well. 
\item It seems like I trained GANs for 1000 epochs while you trained VAEs for 10000. This causes some implicit differences in the evaluation metrics (like VAEs are always better), shall we say something about it? 
\item Read through the appendix
\begin{comment}

\item Decide on the disentanglement metric. Read the following papers (links included):        
    \begin{itemize}
    \item \href{https://openreview.net/pdf?id=Sy2fzU9gl}{BetaVAE metric} cited in \href{https://arxiv.org/pdf/1903.11260.pdf}{Small Data Challenges in Big Data Era}, section Disentanglement Metric page 8
    \item \href{https://arxiv.org/pdf/1905.13662.pdf}{On the fairness of disentangled representations} - The authors said at NeurIPS that the most reliable metric is DCI
    \item Potentially also \href{https://arxiv.org/pdf/1905.12506.pdf}{Are Disentangled Representations Helpful for Abstract Visual Reasoning?} - on their poster it looked like they compared many different ones using VAEs, might be relevant
    \end{itemize}

\item Decide on IS and FID score, do we want to implement both? Read the following papers (links included):
    \begin{itemize}
        \item \href{https://arxiv.org/pdf/1901.01091.pdf}{Adaptive Density Estimation for GMs} - see Table 3 for different score benchmarks. The IS and FID metrics are explained and referenced in Appendix D. Also, the authors claimed at their poster that they learned disentangled representations but they didn't do any study on that in the paper.
    \end{itemize}
\end{comment}
    

\end{itemize}
\begin{comment}
\Large{
$\textbf{g}$
\\
${\color{orange}\{\tau = g(\alpha) \,|\, \alpha_l = I_d \}}$ \\
${\color{teal}\{\tau\,|\,\tau \sim p(\tau) \}}$
\\
$\textbf{Env}$
\\
${\color{orange}\boldsymbol{S}_g^{l-Id} = \{s_g^1, \dots, s_g^n\}}$ \\
${\color{teal}\boldsymbol{S}_r = \{s_r^1, \dots, s_r^n\}}$
\\
$\boldsymbol \proj_j$
\\
${\color{orange}\proj_j \boldsymbol{S}_g^{l-Id} = \{\proj_j s_g^1, \dots, \proj_j s_g^n\}}$ \\
${\color{teal}\proj_j \boldsymbol{S}_r = \{\proj_j s_r^1, \dots, \proj_j s_r^n\}}$

$\MMD(\proj_j \boldsymbol{S}_g^{l-Id}, \proj_j \boldsymbol{S}_r)$
\\
{\color{gray} phase 1} \\
{\color{gray} phase 2}}
\end{comment}
